Classifying Conspiratorial Narratives At Scale: False Alarms and Erroneous Connections

Online discussions frequently involve conspiracy theories, which can contribute to the proliferation of belief in them. However, not all discussions surrounding conspiracy theories promote them, as some are intended to debunk them. Existing research has relied on simple proxies or focused on a constrained set of signals to identify conspiracy theories, which limits our understanding of conspiratorial discussions across different topics and online communities. This work establishes a general scheme for classifying discussions related to conspiracy theories based on authors' perspectives on the conspiracy belief, which can be expressed explicitly through narrative elements, such as the agent, action, or objective, or implicitly through references to known theories, such as chemtrails or the New World Order. We leverage human-labeled ground truth to train a BERT-based model for classifying online CTs, which we then compared to the Generative Pre-trained Transformer machine (GPT) for detecting online conspiratorial content. Despite GPT's known strengths in its expressiveness and contextual understanding, our study revealed significant flaws in its logical reasoning, while also demonstrating comparable strengths from our classifiers. We present the first large-scale classification study using posts from the most active conspiracy-related Reddit forums and find that only one-third of the posts are classified as positive. This research sheds light on the potential applications of large language models in tasks demanding nuanced contextual comprehension.

==> 100_checklist.tex <==


\section{Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}

    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?

    \answerYes{Answer: Yes, and we verified that our research 1) does not violate privacy norms or unfair profiling (Sec.9, under ``User Anonymity and Privacy"), 2) is not tied to any socio-economic factors, 3) does not imply disrespect to societies or cultures (Sec.9, under ``Content Credibility").}
    %\answerYes{Answer: Yes, and as described in the introduction (Sec.1), our research questions focus on the classification of conspiracy theories in online discussions. While our study does advance scientific understanding in the domain of natural language processing and information classification, we have been mindful of potential ethical concerns and social contracts throughout our research process. Firstly, our research does not violate privacy norms or perpetuate unfair profiling. We do not target individuals but rather analyze publicly available content on online forums. We respect the privacy of users and do not collect or use personally identifiable information. Secondly, our study does not exacerbate socio-economic divides. Our analysis of online discussions is not tied to any socio-economic factors, and our findings aim to provide insights into the prevalence of conspiracy theories across different online communities, fostering a better understanding of online discourse. Lastly, our research does not imply disrespect to societies or cultures. While presenting conspiracy narratives for illustrative purposes in our paper, we acknowledge the potential that some readers may consider them credible. It is important to emphasize that we have not conducted fact-checks to verify the accuracy of these narratives, we maintain a neutral stance while analyzing and classifying conspiracy theories, and our goal is to contribute to a more nuanced understanding of online discussions without judgment or bias. Our research seeks to advance science in a responsible and ethical manner, respecting social contracts, privacy norms, and cultural sensitivities. Our findings aim to shed light on online discourse and contribute to informed discussions about conspiracy theories without perpetuating harm or inequality.}
    
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
  
    \answerYes{Answer: Yes, and as described in the abstract, we introduce a comprehensive scheme (Sec.3 and 5) for classifying conspiracy theories on Reddit (Sec.4), we leverage BERT-based models to build conspiracy theory classifiers and compare their performance to Generative Pre-trained Transformer (GPT) (Sec.6 and 7) while identifying its shortcomings (Sec.7.2). We also present the first large-scale classification study of conspiracy-related Reddit forums (Sec.7.3)}
    
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
   
    \answerYes{Answer: Yes. We discussed the limitations of existing methods (Sec.1 and 2) and proposed a classification scheme followed by hired and trained human annotators (Sec.3, and 5). We targeted the most popular online forums. We employed a diverse set of machine learning techniques, including both traditional and advanced deep learning methods, along with the GPT (Sec.6). In particular, these models have been extensively explored in prior research, showcasing their remarkable expressiveness and aptitude for understanding textual language. This solid foundation in the literature substantiates our rationale for incorporating these models into our study.}
    
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
   
    \answerYes{Answer: Yes, and it can be found in ``Ethical Consideration" (Sec.9) section, under ``Data Collection and Management".}
    
  \item Did you describe the limitations of your work?
  
    \answerYes{Answer: Yes, and it can be found in the ``Discussion" (Sec.8) and ``Ethical Consideration" (Sec.9) sections.}
    
  \item Did you discuss any potential negative societal impacts of your work?
  
    \answerYes{Answer: Yes, and it can be found in ``Ethical Consideration" (Sec.9) section, under ``Content Credibility" and ``Potential Impacts of Work".}
      
      \item Did you discuss any potential misuse of your work?
      
    \answerYes{Answer: Yes, and it can be found in ``Ethical Consideration" (Sec.9) section, under ``Potential Impacts of Work".}
    
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    
    \answerYes{Answer: Yes, and it can be found in ``Ethical Consideration" (Sec.9) section, under ``User Anonymity and Privacy" and ``Potential Use/Abuse of Work".}
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  
    \answerYes{Answer: Yes, and we adhere to the guidelines, as demonstrated in Sec.9.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
  
    \answerNA{Answer: NA}
    
  \item Have you provided justifications for all theoretical results?
  
    \answerNA{Answer: NA}
    
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
  
    \answerNA{Answer: NA}
    
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
  
    \answerNA{Answer: NA}
    
  \item Did you address potential biases or limitations in your theoretical framework?
  
    \answerNA{Answer: NA}
    
  \item Have you related your theoretical results to the existing literature in social science?
  
    \answerNA{Answer: NA}
    
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
  
    \answerNA{Answer: NA}
    
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
  
    \answerNA{Answer: NA}
    
	\item Did you include complete proofs of all theoretical results?
 
    \answerNA{Answer: NA}
    
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  
    \answerNo{Answer: No, because access to data via third-party services was limited per Reddit's introduction of new Data API (Please refer to Sec.9, under ``Data Collection and Management"). We adhere to Reddit's new policy and the platform's data usage guidelines.}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  
    \answerYes{Answer: Yes, and the details can be found in Sec.6.}
    
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
     
    \answerNo{Answer: No, due to space constraints. While we conducted thorough experiments encompassing various Machine Learning models with diverse text embeddings, we were constrained by space and thus could only present the best result for each tested setting in Sec.7. However, most of the experiments listed in the paper utilized default parameters, and our hyperparameter search was limited, as stated in Sec.6.}
    
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
 
    \answerYes{Answer: Yes, and it can be found in Sec.6.}
    
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made?
     
    \answerYes{Answer: Yes, and it can be found in Sec.7.}
    
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
     
    \answerYes{Answer: Yes, and it can be found in Sec.7.2.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  
    \answerYes{Answer: Yes, we have provided proper citations for all the used assets and models.}
    
  \item Did you mention the license of the assets?
  
    \answerNo{Answer: No, because the images and tables featured in the paper were generated by the authors. Any software and reused codes utilized in this study are open source.}
    
  \item Did you include any new assets in the supplemental material or as a URL?
  
    \answerNo{Answer: No, because we do not provide supplement materials. Publishing our assets is subject to Reddit's permission (please refer to answer 4.a in this checklist and Sec.9).}
    
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  
    \answerYes{Answer: Yes, and it can be found in Sec.9 under ``Data Collection and Management".}
    
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  
    \answerYes{Answer: Yes, and it can be found in Sec.9 under ``Data Collection and Management".}
    
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?

\answerNo{Answer: No, because we do not share the dataset at the time (please refer to answer 4.a in this checklist and Sec.9). Our dataset includes metadata that adheres to the principles of FAIR. It will be made available to the public following approval from Reddit. }

\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 

\answerYes{Answer: Yes, and it will be published along with the dataset (subject to Reddit's permission, refer to Sec.9).}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
  
    \answerNA{Answer: NA}
    
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
  
    \answerNA{Answer: NA}
    
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  
    \answerNA{Answer: NA}
    
   \item Did you discuss how data is stored, shared, and deidentified?
   
   \answerNA{Answer: NA}
   
\end{enumerate}

\end{enumerate}



